Ridge Rider: Finding Diverse Solutions by Following Eigenvectors of the Hessian

Over the last decade, a single algorithm has changed many facets of our lives - Stochastic Gradient Descent (SGD). In the era of ever decreasing loss functions, SGD and its various offspring have become the go-to optimization tool in machine learning and are a key component of the success of deep neural networks (DNNs). While SGD is guaranteed to converge to a local optimum (under loose assumptions), in some cases it may matter which local optimum is found, and this is often context-dependent. Examples frequently arise in machine learning, from shape-versus-texture-features to ensemble methods and zero-shot coordination. In these settings, there are desired solutions which SGD on 'standard' loss functions will not find, since it instead converges to the 'easy' solutions. In this paper, we present a different approach. Rather than following the gradient, which corresponds to a locally greedy direction, we instead follow the eigenvectors of the Hessian, which we call "ridges". By iteratively following and branching amongst the ridges, we effectively span the loss surface to find qualitatively different solutions. We show both theoretically and experimentally that our method, called Ridge Rider (RR), offers a promising direction for a variety of challenging problems.

==> conclusion.tex <==

\section{Conclusion and Future Work}



==> core/5_experiments_full.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate \accmethod{} in the following settings: exploration in RL, zero-shot coordination, and supervised learning on both MNIST and the more challenging Colored MNIST problem \cite{arjovsky2019invariant}. In the following section we introduce each of the settings and present results in turn.

\subsection{ \method{} for Diversity in Reinforcement Learning}
\label{subsection:diversityrr}

To test whether we can find diverse solutions in RL, we use a toy binary tree environment with a tabular policy. The agent begins at $s_1$, selects actions $a\in \{\mathrm{left}, \mathrm{right}\}$, receiving reward $r \in \{-1, 10\}$ upon reaching a terminal node. The composition of the trees (example in Fig~\ref{fig:tree_results}) is such that there are more negative terminal nodes than positive ones. This makes it less likely for an agent to discover high reward nodes deeper in the tree, as going deeper increases the probability of a negative reward. For the loss function, we compute the expectation of a policy as the sum of the rewards of each terminal node, weighted by the cumulative probability of reaching that node. The maximum reward is $10$. 


We use the exact version of \accmethod{} and find $\theta^\text{MIS}$, by maximizing entropy. For the $\mathrm{ChooseFromArchive}$ precedure, we use BFS. Since we use a tabular policy, we have access to exact gradients, and we can cheaply re-compute the Hessian and EVecs. As such, when we call $\mathrm{UpdateRidge}$ we adapt the learning rate $\alpha$ online to take the largest possible step while preserving the ridge. We begin with a large $\alpha$, take a step, recompute the EVecs of the Hessian and the maximum overlap $\delta$. We then and sequentially halve $\alpha$ until we find a ridge satisfying the $\delta_\mathrm{break}$ criteria (or $\alpha$ gets too small). 
In addition, we use the following criteria for $\mathrm{EndRide}$: (1) If the dot product between $e_i$ and $e'_i$ is less than $ \delta_{\text{break}}$ (2) If the policy stops improving. 
%In experiments we demonstrate that the approach described is an effective way to find diverse solutions, but also note the potential 

\vspace{-2mm}
\begin{figure}[H]
        \resizebox{2.5cm}{!}{\centering\begin{tikzpicture}
            \tikzstyle{VertexStyle}=[decision]
            \Vertex[L=$s_1$,x=2,y=0]{X}
            
            \Vertex[L=$s_2$,x=1.3,y=-0.7]{A}
            \tikzstyle{VertexStyle}=[reward]
            \Vertex[L=$+$,x=0.9,y=-1.4]{Y}
            \tikzstyle{VertexStyle}=[badreward]
            \Vertex[L=$-$,x=1.6,y=-1.4]{Z}
            
            \tikzstyle{VertexStyle}=[decision]
            \Vertex[L=$s_3$,x=2.7,y=-0.7]{B}
            \tikzstyle{VertexStyle}=[badreward]
            \Vertex[L=$-$,x=2.3,y=-1.4]{C}            
            \tikzstyle{VertexStyle}=[decision]
            \Vertex[L=$s_4$,x=3.1,y=-1.4]{D} 
            
            \tikzstyle{VertexStyle}=[decision]
            \Vertex[L=$s_5$,x=2.7,y=-2.1]{E}
            \tikzstyle{VertexStyle}=[badreward]
            \Vertex[L=$-$,x=3.5,y=-2.1]{F}
            
            \tikzstyle{VertexStyle}=[decision]
            \Vertex[L=$s_6$,x=2.3,y=-2.8]{G}
            \tikzstyle{VertexStyle}=[reward]
            \Vertex[L=$+$,x=3.1,y=-2.8]{H}
            
            \tikzstyle{VertexStyle}=[reward]
            \Vertex[L=$+$,x=1.9,y=-3.5]{I}
            \tikzstyle{VertexStyle}=[badreward]
            \Vertex[L=$-$,x=2.7,y=-3.5]{J}
            %\AddVertexColor{blue!30}{D, F, H}
            %\AddVertexColor{red!30}{E, G}
            \AssignVertexLabel{D}{1}
            
            \Edges(A, X,B)
            \Edges(Y, A, Z)
            \Edges(C, B, D)
            \Edges(E, D, F)
            \Edges(G, E, H)
            \Edges(I, G, J)

        \end{tikzpicture}}
        \qquad
        \begin{minipage}{0.78\textwidth}
        \vspace{-30mm}
        \centering\includegraphics[width=0.99\linewidth]{plots/tabular_tree/rr_rl_main.pdf}
        \end{minipage}
        \caption{\textbf{Left}: a tree with six decision nodes and seven terminal nodes, four of which produce negative rewards (red) and three of which produce positive rewards (blue). \textbf{Right}: The percentage of solutions found per algorithm, collated by tree depth. R and S represent starting from a random position or from a saddle, respectively. Trees at each depth are randomly generated $20$ times to produce error estimates shown.}
        \label{fig:tree_results}
\end{figure}
\vspace{-4mm}

We run \accmethod{} with a maximum budget of $T=10^5$ iterations  similarity $\delta_\mathrm{break}=0.95$, and take only the top $N=6$ in $\mathrm{GetRidges}$. As baselines, we use gradient descent (GD) with random initialization, GD starting from the MIS, and random norm-one vectors starting from the MIS. All baselines are run for the same number of timesteps as used by \accmethod{} for that tree. For each depth $d\in \{4,6,8,10\}$ we randomly generate $20$ trees and record the percentage of positive solutions found. 



The results, presented on the right hand side of Fig~\ref{fig:tree_results}, show that \accmethod{} outperforms all three baselines. While \accmethod{} often finds over $90\%$ of the solutions, GD finds at most $50\%$ in each setting. Importantly, following random EVecs performs poorly, indicating the importance of using the EVecs to explore the parameter space. To run this experiment, see the notebook at \url{https://bit.ly/2XvEmZy}.

\begin{comment}
\begin{wrapfigure}{r}{0.5\textwidth} 
\vspace{-5mm}
    \centering\begin{minipage}{0.5\textwidth}
    \centering\subfigure{
        % \includegraphics[width=0.99\linewidth]{plots/tabular_tree/tree_ridges3.png}
        \includegraphics[width=0.65\linewidth]{plots/tabular_tree/optimization_path_few.pdf}    
    } 
    \end{minipage}
    \vspace{-3mm}
    \caption{\small{Example optimization paths. Dark is higher reward. All methods start at the same saddle. The deterministic GDs follow the same trajectory while the RRs follow different paths.}}
    \vspace{-8mm}
    \label{fig:rr_path}
\end{wrapfigure}
\end{comment}

To illustrate this exploration, the left hand side of Fig~\ref{fig:rr_rl_ablation} shows the path along two ridges for the tree shown in Fig~\ref{fig:tree_results}. Areas of high reward are in dark blue. The ridges (green and light blue) both correspond to distinct positive solutions. The policies have six dimensions, but we project them into two dimensions by forming a basis with the two ridges.
%To view the parameters in two dimensions, we project them onto the ridges by taking the dot product. 
Observe that the two ridges are initially orthogonal, following the $(x,y)$ axes. Conversely, we also show two runs of GD from the same initialization, each of which find the same solution and are indistinguishable in parameter space.

\vspace{-2mm}
\begin{figure}[H]
        \begin{minipage}{0.99\textwidth}
        %\subfigure{\includegraphics[width=0.3\linewidth]{plots/tabular_tree/optimization_path_few.pdf}} 
        %\subfigure{\includegraphics[width=0.7\linewidth]{plots/tabular_tree/rr_rl_ablation.pdf}} 
         \includegraphics[width=0.3\linewidth]{plots/tabular_tree/optimization_path_few.pdf} 
     \includegraphics[width=0.7\linewidth]{plots/tabular_tree/rr_rl_ablation.pdf}
        \end{minipage}
        \caption{\textbf{Left}: Example optimization paths. Dark is higher reward. All methods start at the same saddle. The deterministic GDs follow the same trajectory while the RRs follow different paths. \textbf{Right}: The percentage of solutions found per algorithm, collated by tree depth. Trees at each depth are randomly generated $20$ times to produce error estimates shown.}
        \label{fig:rr_rl_ablation}
\end{figure}
\vspace{-4mm}

We also must consider whether we need to adapt $\alpha$, the size of the step along the ridge. In larger scale settings this may not be possible, so we now consider the two following ablations:
\begin{enumerate}
    \item \textit{Fixed + UpdateRidge}: Here we continue to update the ridge, but use a fixed $\alpha$.
    \item \textit{Fixed + FixedRidge}: We not only keep a fixed $\alpha$ but also do not update the ridge. Thus, we take repeated small steps along the original ridge until we meet the $\mathrm{EndRide}$ condition.
\end{enumerate}




In both cases we use $\alpha=0.1$, the same value used for the Gradient Descent and Random Vector baselines in Fig. \ref{fig:tree_results}. As we see in Fig. \ref{fig:rr_rl_ablation}, as we impose greater rigidity, the performance declines. However, the results for the fixed ridge are still stronger than any of the baselines from Fig. \ref{fig:tree_results}, showing the power of the original ridges in finding diverse solutions. 


It is also possible to scale our method to the deep RL paradigm. For on-policy methods we can compute $\mathcal{H}$ accurately via the DiCE operator \cite{dice, loaded_dice}. As a first demonstration of this, we consider the same tree problem shown in Fig. \ref{fig:tree_results}, with the same tabular/linear policy. However, instead of computing the loss as an expectation with full knowledge of the tree, we sample trajectories by taking stochastic actions of the policy in the environment. We then compute the Loaded DiCE objective, using a value function, represented by a vector of values. We use the same maximum budget of $T=10^5$, but using $100$ samples to compute the loss function. For  \method{} we alternate between stepping along the ridge and updating the value function (with SGD), while for the baseline we optimize a joint objective. Both \accmethod{} and the baseline use the Loaded DiCE \cite{loaded_dice} loss function for the policy. For RR, we use the adaptive $\alpha$ from the exact setting. The results are shown in Fig. \ref{fig:dice_rl}.

\begin{wrapfigure}{r}{0.45\textwidth} 
        \vspace{-5mm}
        \begin{minipage}{0.45\textwidth}
        \centering{\includegraphics[width=0.9\linewidth]{plots/tabular_tree/rr_rl_approx.pdf}} 
        \end{minipage}
        \caption{The percentage of solutions found per algorithm, collated by tree depth. Trees at each depth are randomly generated $10$ times to produce error estimates shown.}
        \label{fig:dice_rl}
\end{wrapfigure}

For tree depths of four and six, \accmethod{} significantly outperforms the vanilla actor critic baseline, with gains also coming on larger trees. It is important to caveat that these results remain only indicative of larger scale performance, given the toy nature of the problem. However, it does show it is possible to follow ridges when the Hessian is computed with samples, thus, we believe it demonstrates the \emph{potential} to scale  \method{} to the problems we ultimately wish to solve. 

%Rather than following the gradient, \accmethod{} follows the eigenvectors of the Hessian. The intuition behind \accmethod{} is that of a hiker on the top of the mountain. Is it better to take the steepest path down the cliff or instead pursue the more gently sloping ridge to get to the bottom of the hill? While the answer is problem specific, being able to explore many paths down is valuable. 



%Over the last decade, a single algorithm has dominated the machine learning world - Stochastic Gradient Descent (SGD). Thanks to the increasing capability of deep neural networks (DNNs), SGD and its offspring have become the go-to approach for optimizing losses in machine learning.

%However, while SGD applied to DNNs can reliably return a solution with low loss, there are currently no methods that allow for a systematic exploration of the solution space. In practice, we care greatly about the type of solution obtained; For example, when learning an image classifier, those solutions relying on shape features are known to generalize much better than those relying on textures\cite{DBLP:journals/corr/abs-1811-12231}. 

%\todo{Alex:I think this should go in related work, not in intro} Many methods~\cite{novelty, vime, burda2018exploration, pathak} address this issue by augmenting the loss function. They combine the traditional objective, such as reward in Reinforcement Learning (RL), with some form of \emph{bonus} to explore the solution space. While successful in achieving the targeted goal, this way of incorporating a prior into the model further restricts the possible solution space. Coupled with SGD, the result is a beeline for a particular solution to the augmented objective, which may not actually be the best one.

%In this paper, we present a fundamentally different approach called \emph{ \method{}} (RR). Rather than following the gradient, \accmethod{} follows the eigenvectors of the Hessian. The intuition behind \accmethod{} is that of a hiker on the top of the mountain. Is it better to take the steepest path down the cliff or instead pursue the more gently sloping ridge to get to the bottom of the hill? While the answer is problem specific, being able to explore many paths down is valuable. 


%Consider the example of a binary tree, shown in Fig. \ref{fig:binarytree}. The agent begins at $s_0$ and must decide whether to go $\mathrm{left}$ or $\mathrm{right}$ at each node. Three terminal states provide a positive reward, while the rest return a negative reward. It is clear to see that the positive rewards at higher levels of the tree are significantly easier to find. Using a tabular policy, and taking gradients with respect to the expected reward (by computing weighted probabilities for each leaf node), we only achieve the first solution.


%Now consider the case where the reward function may not be perfectly specified. For instance, there may be some other desirable property which makes makes the more challenging solutions more valuable. In this case, the inability of SGD to recover this solution becomes a critical issue. We believe this problem will only increase as the machine learning community shifts away from well-specified loss functions. We see this problem clearly in many settings \cite{Geirhos2020a,DBLP:journals/corr/abs-1811-12231}, two of which are zero-shot coordination and computer vision. 

%In the coordination setting, deploying a strategy that is unique is more likely to lead to success than picking one arbitrary policy out of many equivalent, but mutually incompatible policies. With just the self-play objective, SGD will not distinguish the `uniqueness' of the solution and will instead arbitrarily maximize the objective function. A real-world example of this is trying to find someone in New York without prior planning. For our purposes, we adapt the lever coordination game from \cite{hu2020other} to highlight how \accmethod{} finds a more amenable solution than SGD.

%In computer vision, we would prefer to find solutions which rely on semantic characteristics because those are much more capable for downstream tasks. However, most DNNs instead find solutions based on texture instead of shape. This leads to problems exemplified by finding a sheep in an empty meadow \cite{Geirhos2020a}.

%More generally, being able to find a variety of solution classes has practical implications for RL and ensemble methods, where it can help produce more robust results.


% A canonical example of this issue is when trying trying to coordinate with a stranger in a Zero-Shot setting, deploying a strategy that is unique of its type is more likely to lead to success than picking one arbitrary policy out of many equivalent, but mutually incompatible, policies. With just the value of the self-play objective, SGD will not distinguish the ``uniqueness'' of the solution, and will instead arbitrarily maximize the objective function. 

% Being able to change the type of solution being learned also has practical implications for Reinforcement Learning and ensemble methods, where it can help produce more robust results.

\subsection{ \method{} for Supervised Learning}

Our main findings for approximate \accmethod{} applied to MNIST are as follows:
\begin{enumerate}
    \item We can achieve respectable performance of approximately $98\%$ test and train accuracy with a 2-layer MLP containing 128 dimensions in the hidden layer. See the left hand side of Fig~\ref{fig:mnist_training} for training curves and hyperparameters.
    \item Updating $e$ to follow the changing eigenvector is crucial. A simple ablation which sets LR$_{e}$ to 0 fails to train beyond $90\%$
    on MNIST, even after a large hyper parameter sweep. See the right side of Fig~\ref{fig:mnist_training}. 
    \item With fixed hyperparameters and initialization, the order in which the digit classes are learned changes according to the fingerprint. This is seen in Figure~\ref{fig:mnist_diversity}. The ridges with low indices (i.e. eigenvectors with very negative curvature) correspond to learning `0' and `1' initially, the intermediate ridges correspond to learning `2' and `3' first, and the ridges at the upper end of the spectrum we sampled (ie. $>30$) correspond to learning features for the digit ``8''.
\end{enumerate}


 
 \begin{comment}
  \begin{figure*}[ht]
    \centering
    %\includegraphics[width=0.5\textwidth]{plots/with_without_ridge.pdf}
    % \includegraphics[width=0.5\textwidth]{plots/mnist.pdf}
    \includegraphics[width=0.4\textwidth]{plots/with_without_ridge_trim.pdf}
    \caption{We compare a hyperparameter sweep for approximate \accmethod{} on MNIST with a simple ablation: Rather than updating the ridge (EVec), we set LR$_e$ to 0, i.e. keep following the original direction of the EVec. Shown are the runs that resulted in over $>60\%$ final test accuracy out of a hyper parameter sweep over 2000 random trials. We note that updating the ridge is absolutely crucial of obtaining high performance on MNIST - simply following the fixed eigenvectors with an otherwise unchanged \accmethod{} algorithm never exceeds the performance of a linear classifier.}
    \label{fig:mnist_with_without_ridge}
\end{figure*}
\end{comment}

 \begin{figure*}[ht]
    \centering
    \includegraphics[width=0.34\textwidth]{plots/mnist.pdf}
    % \includegraphics[width=0.33\textwidth]{plots/with_without_ridge_trim.pdf}
    \includegraphics[width=0.33\textwidth]{plots/ablation_mnist.pdf}
    \caption{\textbf{Left}: Test and training accuracy on MNIST. Our hyperparameters for this experiment were: $S=236$, $\alpha=0.00264$, $\text{LR}_x~=0.000510$, $\text{LR}_\lambda=4.34e^{-6}$, $\text{batch size}=2236$. \textbf{Right}: We compare a hyperparameter sweep for approximate \accmethod{} on MNIST with a simple ablation: Rather than updating the ridge (EVec), we set LR$_e$ to 0, i.e. keep following the original direction of the EVec. Shown are the runs that resulted in over $>60\%$ final test accuracy out of a hyper parameter sweep over 2000 random trials. We note that updating the ridge is absolutely crucial of obtaining high performance on MNIST - simply following the fixed eigenvectors with an otherwise unchanged \accmethod{} algorithm never exceeds the performance of a linear classifier.}
    \label{fig:mnist_training}
\end{figure*}
% \vspace{-6mm}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{plots/diversity_n.pdf}
    \includegraphics[width=\textwidth]{plots/diversity_later_n.pdf}
    \caption{Class accuracy for different digits as a function of the index of the first ridge ($\psi[0]$), i.e the ranking of the EVal corresponding to the first EVec we follow. \textbf{Top}: Early in training -- average between $200$ and $600$ steps. \textbf{Bottom}: Later in training, averaged between $4000:5000$ steps. The architecture is the same MLP as in Figure~\ref{fig:mnist_training}, but the hyperparameters are: $S=1$, $\alpha=0.000232$, $\text{LR}_x=3.20e^{-6}$, $LR_\lambda=0.00055$, $\text{batch size}= 2824$.}
    \label{fig:mnist_diversity}
\end{figure*}

 

\subsection{ \method{} for Zero-Shot Coordination}

We test \accmethod{} as described in Sec \ref{subsection:zeroshotrr} on multi-agent learning using the lever coordination game from~\citet{hu2020other}. The goal is to maximize the expected reward $J$ when playing a matrix game with a stranger. On each turn, the two players individually choose from one of ten levers. They get zero reward if they selected different levers and they get the payoff associated with the chosen lever if their choices matched. Importantly, not all levers have the same payoff. In the original version, nine of the ten levers payed $1$ and one paid $.9$. In our more difficult version, seven of the ten levers pay $1$, two `partial coordination' levers pay $0.8$, and one lever uniquely pays $0.6$. In self-play, the optimal choice is to pick one of the seven high-paying levers. However, since there are seven equivalent options, this will fail in zero-shot coordination. Instead, the optimal choice is to pick a lever which obtains the highest expected payoff when paired with any of the equivalent policies. Like in the RL setting, we use a BFS version of exact \accmethod{} and the MIS is found by optimizing for high entropy and low gradient.

% \vspace{-1mm}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/matrix_game/runs_payoffs_errorbars.flipped.scale3.pdf}
    \caption{Zero-Shot Coordination: On the left, we see the average payoff per ridge over 25 runs, repeated five times to yield error estimates. As expected, the highest payoff is $0.6$ and it occurs when both agents find the symmetry breaking solution, even though that solution yields the lowest payoff in self-play. On the right, we see the results of three randomly chosen runs where each square is a probability that \emph{one} of the two agents select that action. We verified that the agents in each run and each ridge agree on the greedy action.}
    \label{fig:matrix_game}
\end{figure*}

We see in Fig~\ref{fig:matrix_game} that \accmethod{} is able to find each solution type: the self-play choices that do poorly when playing with others (ridges 1, 3-5, 7-9), the `partial coordination' that yield lower reward overall (ridges 2 and 6), and the ideal coordinated strategy (ridge 0). Note that based on this protocol the agent will chose the $0.6$ lever, achieving perfect zero-shot coordination.\footnote{To run the zero-shot coordination experiment, see the notebook at \url{https://bit.ly/308j2uQ.}}



% \paragraph{Supervised Learning} Finally, we show results on MNIST\cite{lecun2010mnist} and Colored MNIST\cite{arjovsky2019invariant}. 

% Our results on MNIST are meant to highlight that \accmethod{} can achieve respectable results in supervised learning on a straightforward task where there is only one acceptable minimum. Accordingly, we achieve \cinjon{todo: fill in accuracy + confidence over five seeds} with hyperparameters specified in the appendix. More interestingly, we also see in Fig~\ref{mnist_filters} \cinjon{todo: insert the filters} that the Hessian eigenvectors are themselves indicative of the digits.

\subsection{ \method{} for Out of Distribution Generalization} We test our extension of \accmethod{} from Sec \ref{subsec:OOD} on OOD generalization using Colored MNIST \cite{arjovsky2019invariant}. Following Sec~\ref{subsection:oodg}, for each of $\xi_{1, 2}$ in $\Xi$, as well as test environment $\xi_3$, $x_i \in D_{\xi_k}$ are drawn from disjoint subsets of MNIST \cite{lecun2010mnist} s.t. $|D_{\xi_{1, 2}}| = 25000$ and $|D_{\xi_{3}}| = 10000$. Further, each has an environment specific $p_{\xi_k}$ which informs $\mathcal{D}_{\xi_k}$ as follows: For each $x_i \in D_{\xi_k}$, first assign a preliminary binary label $\tilde{y_i}$ to $x_i$ based on the digit -- $\tilde{y_i} = 0$ for $x_i \in [0,4]$ and $\tilde{y_i} = 1$ for $x_i \in [5,9]$. The actual label $y_i$ is $\tilde{y_i}$ but flipped with probability $.25$. Then, sample color id $z_i$ by flipping $y_i$ with probability $p_{\xi_k}$, where $p_{\xi_1}=0.2$, $p_{\xi_2}=0.1$, and $p_{\xi_3}=0.9$. Finally, color the image red if $z_i = 1$ or green if $z_i = 0$.  Practically, we first optimize $\mathcal{L}_1+\mathcal{L}_2$ to find the MIS, resampling the DNN when optimization fails to obtain a low loss.

\begin{wraptable}{r}{5.5cm}
\vspace{-8mm}
\begin{tabular}{c|c|c}
Method & Train Acc & Test Acc \\
\toprule
\textbf{RR} & $65.5 \pm 1.68$ & $58.4 \pm 2.41$ \\
ERM & $87.4 \pm 1.70$ & $17.8 \pm 1.33$ \\
IRM & $69.7 \pm .710$ & $65.7 \pm 1.42$ \\
\toprule
Chance & $50$ & $50$ \\
Optimal & $75$ & $75$ \\
\end{tabular}
\vspace{-1mm}
\caption{\textbf{Colored MNIST}: Accuracies on a $95\%$ confidence interval. \accmethod{} is in line with causal solutions.}
\label{table:colored-mnist}
\vspace{-3mm}
\end{wraptable} 

Chance is $50\%$. The optimal score is $75\%$ on train \emph{and} test. Fitting a neural network with ERM and SGD yields around $87\%$ on train and $18\%$ on test because it only finds the spurious color correlation. Methods which instead seek the more causal digit explanation achieve about $66\%-69\%$\cite{arjovsky2019invariant,ahuja2020invariant,krueger2020outofdistribution}. As shown in Table~\ref{table:colored-mnist}, our results over $30$ runs achieve a high %after seven steps along the ridge of $63.1\% \pm .574$ on train and $57.4\% \pm .608$ on test.
after nine steps along the ridge of $65.5\% \pm 1.68$ on train and $58.4\% \pm 2.41$ on test.
\footnote{To run the out of distribution generalization experiment, see the notebook at \url{https://bit.ly/3gWeFsH.}} Our results are clearly both above chance and in line with models that find the causal explanation rather than the spurious correlative one. See Fig~\ref{fig:colored_mnist} in the Appendix for graphs.




==> theory.tex <==
\section{Theoretical Results}


